Adversarial Pixel Restoration as a Pretext Task for Transferable Perturbations

Transferable adversarial attacks optimize adversaries from a pretrained surrogate model and known label space to fool the unknown black-box models. Therefore, these attacks are restricted by the availability of an effective surrogate model. In this work, we relax this assumption and propose Adversarial Pixel Restoration as a self-supervised alternative to train an effective surrogate model from scratch under the condition of no labels and few data samples. Our training approach is based on a min-max scheme which reduces overfitting via an adversarial objective and thus optimizes for a more generalizable surrogate model. Our proposed attack is complimentary to the adversarial pixel restoration and is independent of any task specific objective as it can be launched in a self-supervised manner. We successfully demonstrate the adversarial transferability of our approach to Vision Transformers as well as Convolutional Neural Networks for the tasks of classification, object detection, and video segmentation. Our training approach improves the transferability of the baseline unsupervised training method by 16.4% on ImageNet val. set. Our codes & pre-trained surrogate models are available at: https://github.com/HashmatShadab/APR

==> figures/attention_maps_main_paper.tex <==
\begin{figure*}[!t]
\begin{minipage}{0.5\textwidth}
  
\centering
\begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
    \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/input_image1.jpeg}
  \end{minipage}
  \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
   \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/clean/1.png}
  \end{minipage}
\begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up
  \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/baseline/1.png}
  \end{minipage}
     \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
    \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/ours/1.png}
  \end{minipage}
  \\
  \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
    \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/input_image2.jpeg}
  \end{minipage}
  \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
    \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/clean/2.png}
  \end{minipage}
  \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
    \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/baseline/2.png}
  \end{minipage}
    \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
    \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/ours/2.png}
  \end{minipage}
  \\
  \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
     \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/input_image4.JPEG}
     \footnotesize Samples
  \end{minipage}
      \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up
    \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/baseline/4.png}
    \footnotesize Clean Maps
  \end{minipage}
  \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
    \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/baseline/4.png}
    \footnotesize \cite{li2020practical}
  \end{minipage}
   \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up
    \includegraphics[height=1.2cm, width=\linewidth]{images/attn_vis/ours/4.png}
    \footnotesize Ours
  \end{minipage}

  \end{minipage}
  \hfill
  \begin{minipage}{0.48\textwidth}
  \vspace{-1em}
    \caption{ \small GradCAM \cite{selvaraju2017grad} explanation of adversarial examples. The activation maps were generated on ImageNet pretrained ResNet50 model. Adversarial examples are transferred from surrogate  trained via our adversarial rotation restoration task at the perceptual budget of $\epsilon \le 0.1$ \cite{li2020practical}. Our approach significantly shifts the attention of the model, boosting the mis-classifcation rates on the adversarial examples (see Appendix B
    %\ref{appendix: attention dispersion} 
    for more qualitative examples). }
  \label{fig:attn_vis}
  \end{minipage}
  \vspace{-1em}
\end{figure*}
